Product of Orthogonal Spheres Parameterization for Disentangled Representation Learning

Learning representations that can disentangle explanatory attributes underlying the data improves interpretabilty as well as provides control on data generation. Various learning frameworks such as VAEs, GANs and auto-encoders have been used in the literature to learn such representations. Most often, the latent space is constrained to a partitioned representation or structured by a prior to impose disentangling. In this work, we advance the use of a latent representation based on a product space of Orthogonal Spheres PrOSe. The PrOSe model is motivated by the reasoning that latent-variables related to the physics of image-formation can under certain relaxed assumptions lead to spherical-spaces. Orthogonality between the spheres is motivated via physical independence models. Imposing the orthogonal-sphere constraint is much simpler than other complicated physical models, is fairly general and flexible, and extensible beyond the factors used to motivate its development. Under further relaxed assumptions of equal-sized latent blocks per factor, the constraint can be written down in closed form as an ortho-normality term in the loss function. We show that our approach improves the quality of disentanglement significantly. We find consistent improvement in disentanglement compared to several state-of-the-art approaches, across several benchmarks and metrics.

==> Sections/Motivation.tex <==
 We would also like to present a motivation for the choice of orthogonality in latent-spaces by first principles analysis of typical factors of image-formation. An image can be seen as a complex non-linear interaction between various factors such as lighting, pose, shape, and shading. In many cases, there is a wealth of literature that studies the basic geometric properties of each mode of variation. However, it has been found that the specific constraints are too specific for each factor, and generally not compatible with each other, or with contemporary machine learning models. In this section, we show that a slight relaxation of some of these classical findings will lead to a very natural compact model for latent-variables in the form of a product of orthogonal-spheres. This new model is very simple to implement and enforce as a simple loss-function in deep-learning modules. We start with a few common factors in image-formation, and develop the model.
\begin{enumerate}
    \item {\bf Lighting variables: } In the illumination cone model, assuming Lambertian reflectance, and convex object-shapes, one can show that the image space is a convex-cone in image space \cite{Georghiades2001}. A relaxation of this model leads to identifying cones as linear-subspaces, which are seen as points on a Grassmannian manifold $\mathcal{G}_{n,k}$ ($n$ = image-size, $k$ = lighting dimensions, typically considered equal to number of linearly independent normals on the object shape) \cite{Lohit2017}. Under certain conditions of variance on the Grassmannian being low, a distribution of points on the Grassmann induces a distribution on a high-dimensional sphere (see \cite{ChakrabortyICCV2015}), whose dimension depends on $n$ and $k$ \cite{ChakrabortyICCV2015}.  %Thus, we can approximately relate fundamental lighting variables as a point on a suitable spherical manifold. 
    \item {\bf Pose variables: } 3D pose is frequently represented as an element of the special orthogonal group $SO(3)$. For analytical purposes, it is convenient to think of rotations represented by quaternions \cite{quaternions}, which are elements of the 3-sphere $S^3$ embedded in $\mathbb{R}^4$, with the additional constraint of antipodal equivalence. This makes rotations to be identified as points on a real-projective space $\mathbb{R}\mathbb{P}^3$. Real-projective spaces are just a special case of the Grassmannian -- in this case, of 1D sub-spaces in $\mathbb{R}^4$. Using similar result as before \cite{ChakrabortyICCV2015}, from a distribution on quaternions, we can induce a distribution in a higher-dimensional hyperspherical manifold.
    \item {\bf Deformation variables: } Deformation of underlying shape, or non-elastic deformation of image-grid (e.g. due to shape change, expression, or photoshop effects), can be modeled by the framework of diffeomorphic maps from $\mathbb{R}^2$ to $\mathbb{R}^2$. Diffeomorphic maps are continuous, smooth, and invertible maps that warp an image grid. Under additional conditions such as corner-point preservation, a square-root form of the diffeomorphic map can be viewed as a point on a infinite-dimensional Hilbert sphere \cite{Jermyn2012}. The infinite-dimensionality is more a mathematical convenience, but in practice, the dimension of the hypersphere is defined by the image-resolution. 
\end{enumerate}

 Now, the relevant question is whether hyperspherical relaxation is a good model for factors beyond the above? Consider for instance the factors listed in table \ref{table:map_celeba}. Most of the factors listed there are mid-level or semantic factors, rather than analytically definable physical factors. However, to a good degree of approximation such semantic factors can be explained as a result of combinations of low-level physical factors. Wavy hair for instance can be approximately described by deformation variables, makeup can be approximated by lighting variables, etc. While our model specifically is motivated by well-studied tractable factors like illumination, pose, and deformation, our conjecture is that the model is quite flexible and applicable beyond these factors. 

==> Sections/PreviousWork.tex <==

%\paragraph{Autoencoders.}Autoencoders \cite{Hinton2006ReducingTD, Bengio2013RepresentationLA} are encoder-decoder type architectures and have extensively been employed to disentangle features using varied training strategies \cite{Szab2018ChallengesID, Mathieu2016DisentanglingFO, Jha2018DisentanglingFO, Reed2015DeepVA, Makhzani2015AdversarialA}. A typical encoder learns to project high dimensional data to a lower dimensional manifold while the task of the decoder is to precisely map it back to the high dimensional data space. VAEs \cite{Kingma2014AutoEncodingVB} are probabilistic generative modifications of autoencoders wherein it is possible to generate novel unseen images by sampling latent codes from a fixed probability distribution. For VAEs, the points in the latent space are predominantly constrained to follow a Gaussian prior.
%We utilize an autoencoder-type architecture for retrieval of finer and coarser attributes ensuring a potent disentanglement model.

%\paragraph{GANs.}A representative GAN \cite{Goodfellow2014GenerativeAN} model consists of two typical modules: a discriminator whose task is to distinguish between real and fake samples; and a generator which tries to generate fake samples that are indistinguishable from the real ones. During training, both of these individual neural networks compete against each other in a min-max fashion trying to learn the optimal distribution of the data. GANs have successfully established their mantle in the domain of disentangled representations \cite{Chen2016InfoGANIR, Choi2018StarGANUG}.
%Our approach uses the architecture of a GAN to generate real-looking images with varying permutations of separated latent factors of variation. 

Disentangling factors of variation to extract meaningful representations has been an engaging area of interest in the research community since long and has been explored in various contexts of style-transfer for both text \cite{John2018DisentangledRL} and image domains \cite{Gatys2016ImageST}, analogy-making \cite{Reed2015DeepVA} and domain adaptation \cite{Vu2017DomainAM, press2018emerging}. Ruiz \etal \cite{Ruiz2018LearningDR} present a weakly supervised, reference based disentanglement using an auto-encoder setting that is backed up with adversarial modelling to avoid degenerate solutions. Press \etal \cite{press2018emerging} learns disentangling in an unsupervised manner with the idea of domain adaptation using an encoder-decoder architecture. Li \etal \cite{Li2018DisentangledSA} proposed unsupervised sequence modelling approach to disentangle temporally dynamic features from the static ones in audios and videos. Our work in this paper, is aligned in appreciating the idea of disentangling to isolate multiple factors of variation present in image data domains.

Several different approaches have successfully achieved disentangling a single specified attribute while considering the remaining information as one assorted factor. These methodologies have spanned different domains of learning i.e. supervised, semi-supervised and unsupervised techniques. Li \etal \cite{Li2019DisentanglingPF} separates hand pose from other appearance factors via supervised learning. It ensures decorrelation within the two factors by incorporating cycle consistency. \cite{Shu2018DeformingAU} achieves disentangling shape from appearance using unsupervised techniques using canonical and template-based coordinate systems. Mathieu \etal \cite{Mathieu2016DisentanglingFO} and Szab{\'o} \etal \cite{Szab2018ChallengesID} successfully separated one attribute of interest using semi-supervised adversarial training. Jha \etal \cite{Jha2018DisentanglingFO} tackles the issue of degenerate solutions by introducing cycle consistency in VAE-type architecture, thus eliminating adversarial learning. 

While these methods disentangle one specified attribute, disentangling  multiple factors of variation simultaneously is still a challenge. Approaches like \cite{Choi2018StarGANUG} condition the input on a favorable mask of factors to be replicated in the output image. Bouchacourt \etal \cite{Bouchacourt2018MultiLevelVA} proposed group level semi-supervision, not considering i.i.d. sample distributions and showed to generalize well to unseen groups during inference. 

While all these approaches require some level of supervision, several unsupervised approaches like $\beta$-VAE \cite{Matthey2017betaVAELB} is a variant of VAE introduces a weighted KL-divergence term to ensure a restrained information bottleneck for the learned disentangled latent representations. $\beta$-TCVAE \cite{Chen2018IsolatingSO}, a variant of $\beta$-VAE, disintegrates the marginal KL-divergence term into dimension-wise KL-divergence and a total correlation term that exhibits the extent of disentanglement. 
Another variant of $\beta$-VAE called Factor-VAE supports the idea of the latent code distribution to be factorial by introducing a discriminator that differentiates a latent code picked from marginal code distribution from one that is a product of them.
Chen \etal \cite{Chen2016InfoGANIR} tries to achieve mutual information maximization between latent codes and corresponding observations via an additional information regularization in an unsupervised fashion. 
Although it works in an unsupervised fashion, lack of encoder-decode style architecture limits the re-usability of the latent codes of an image. 
We aim to propose a generalized approach that works well on any disentangling model which makes use of factorized latent spaces to enhance the extent of disentanglement with no compromise to the veracity of the image quality.  

\noindent \textbf{Geometry in Deep Learning.} Exploring latent spaces under the lens of geometric awareness not only assists in learning their inherent structure but at the same time paves a way towards more robust and entirely secluded factors of variation. Recent works like \cite{Shao2018TheRG} emphasize on the Riemannian Geometry perspective of latent representations considering discrete analogues of computationally expensive continuous counterparts with novel algorithms for geodesic interpolation, parallel transport of tangent and geodesic shooting on the underlying manifold. Shukla \etal \cite{Shukla2019GeometryOD} has well established a connection between disentanglement and Riemannian geometry of underlying resonance to the manifold. For the purpose of avoiding mode collapse, Bang \etal \cite{Bang2018MGGANSM} incorporates a geometry aware understanding for adversarial training while Li \etal \cite{Li2018MRGANMR} adds a separate geometry-aware regularization term in accordance with the manifold hypothesis. Arvanitidis \etal \cite{arvanitidis2018latent} talks about the underlying geometric representations of low-dimensional latent spaces, learnt by generative models and considers distortions in them by inducing Riemannian metric to improve upon various distance measures and interpolations in contrast to Euclidean metric on latent spaces.
Khnel \etal \cite{Khnel2018LatentSN} discuses non-linear manifold statistical techniques to estimate data statistics in latent spaces of generative models like VAEs and GANs. Brahma \etal \cite{Brahma2016WhyDL} proposes various metrics to measure disentanglement and flattening achieved across layers of deep generative architectures. 

% Our approach is more vigorously powerful as it takes into account statistical independence of multiple factors by imposing orthogonality constraint over different disentangled factors and can be efficiently incorporated within any such factorized disentanglement model.


==> Sections/ProposedApproach.tex <==
\vspace{-0.1cm }
\paragraph{Product of orthogonal spheres as a latent-space model.} We would first like to present a motivation for the choice of orthogonality in latent-spaces by first principles analysis of typical factors of image-formation. An image can be seen as a complex non-linear interaction between various factors such as lighting, pose, shape, and shading. In many cases, there is a wealth of literature that studies the basic geometric properties of each mode of variation. However, it has been found that the specific constraints are too specific for each factor, and generally not compatible with each other, or with contemporary machine learning models. In this section, we show that a slight relaxation of some of these classical findings will lead to a very natural compact model for latent-variables in the form of a product of orthogonal-spheres. This new model is very simple to implement and enforce as a simple loss-function in deep-learning modules. We start with a few common factors in image-formation, and develop the model.
\vspace{-0.3cm}
\begin{figure}[h]
\centering
\includegraphics[width = 0.8\textwidth,keepaspectratio]{images/Selection_049.png}
   \caption{Illustration of proposed Product of Orthogonal Spheres as a latent space model}
\label{fig:model}
\end{figure}
\begin{enumerate}
    \item {\bf Lighting variables: } In the illumination cone model, assuming Lambertian reflectance, and convex object-shapes, one can show that the image space is a convex-cone in image space \cite{Georghiades2001}. A relaxation of this model leads to identifying cones as linear-subspaces, which are seen as points on a Grassmannian manifold $\mathcal{G}_{n,k}$ ($n$ = image-size, $k$ = lighting dimensions, typically considered equal to number of linearly independent normals on the object shape) \cite{Lohit2017}. Under certain conditions of variance on the Grassmannian being low, a distribution of points on the Grassmann induces a distribution on a high-dimensional sphere (see \cite{ChakrabortyICCV2015}), whose dimension depends on $n$ and $k$ \cite{ChakrabortyICCV2015}.  %Thus, we can approximately relate fundamental lighting variables as a point on a suitable spherical manifold. 
    \item {\bf Pose variables: } 3D pose is frequently represented as an element of the special orthogonal group $SO(3)$. For analytical purposes, it is convenient to think of rotations represented by quaternions \cite{quaternions}, which are elements of the 3-sphere $S^3$ embedded in $\mathbb{R}^4$, with the additional constraint of antipodal equivalence. This makes rotations to be identified as points on a real-projective space $\mathbb{R}\mathbb{P}^3$. Real-projective spaces are just a special case of the Grassmannian -- in this case, of 1D sub-spaces in $\mathbb{R}^4$. Using similar result as before \cite{ChakrabortyICCV2015}, from a distribution on quaternions, we can induce a distribution in a higher-dimensional hyperspherical manifold.
    \item {\bf Deformation variables: } Deformation of underlying shape, or non-elastic deformation of image-grid (e.g. due to shape change, expression, or photoshop effects), can be modeled by the framework of diffeomorphic maps from $\mathbb{R}^2$ to $\mathbb{R}^2$. Diffeomorphic maps are continuous, smooth, and invertible maps that warp an image grid. Under additional conditions such as corner-point preservation, a square-root form of the diffeomorphic map can be viewed as a point on a infinite-dimensional Hilbert sphere \cite{Jermyn2012}. The infinite-dimensionality is more a mathematical convenience, but in practice, the dimension of the hypersphere is defined by the image-resolution. 
    
\end{enumerate}

Based on above, we posit, that given an image, potentially influenced by one or more of the above factors, we can represent its latent variables as a point on a product-space of hyperspheres. Between those factors, we further assume statistical orthogonality, as a proxy for physical independence of these fundamental variables. Products of spheres is a generalization of tori geometry. The specification is incomplete without knowing the individual dimensions of the hyperspheres involved. For analytical and computational tractability, we choose to set the dimensions of the spheres to be equal to each other. This, in effect imposes a simple orthonormality constraint on the latent space blocks.
% In this work, we present our approach to improve disentanglement by imposing structure in the latent space. The proposed structure imposes orthonormalality constraint on the aggregated latent space representation of a data point. This in effect forces the code vectors to have least information sharing while forcing them to capture disjoint information.

Given a dataset $\calX = \{\bx_1, \bx_2, \ldots, \bx_m \} $, with $f$ and $g$ representing the encoding and decoding functions respectively such that $\bz = f(\bx)$ and $\bx = g(\bz)$. These functions can either represent a generative model or an autoencoder that is employed for disentangling. The latent space representation is given by $\bZ \in \bbR^{d\times k}=\{\bz^1, \bz^2, \ldots, \bz^k\}$, here $k$ is the number of attributes and $\bz^i \in \bbR^{d}$ represents code vector for each of the attributes. An illustration of the proposed parametrization and update strategy is shown in the Figure \ref{fig:model}. Under the PrOSe model, we would like to enforce orthonormality of $\bZ$ on an average across the entire training-data. That is, for the entire network, we augment the disentanglement loss function with a term penalizing deviations from orthonormality of the latent-space blocks, as:
\begin{align}
    \min_{\theta} \quad \calL_{disentangle} + \calL_{orth},
\end{align}
where, $\calL_{orth}$ is the ortho-normality constraint defined on the stacked matrix of the latent code vectors as columns in $\bZ \in \bbR^{d \times k}=[\bz^1 \bz^2  \ldots,  \bz^k]$, where $k$ is the number of latent code partitions and $d$ is the dimension of the latent code and is given by 
\begin{align}
    \calL_{orth} = \left\lVert \bZ^\top \bZ - \bI \right\rVert^2 _F,
\end{align}
where, $\left\lVert . \right\rVert_F$ is the matrix Frobenius norm. The loss-term includes a summation over training-samples in a given mini-batch, which is not explicitly noted above. 
% In \cite{Mixing_2018}, the disentangling architecture consists of an encoder-decoder network, a discriminator and a classifier. 
% the $\calL_{disentangle}$ loss is composed of three terms and is given by  
% \begin{align}
%     \min _{\theta_{enc}, \theta_{dec}, \theta_c} \max_{\theta_{d}}  \lambda_{m} \calL_{m} +\lambda_{c} \calL_{c} +\lambda_{d} \calL_{d} + \calL_{orth}
% \end{align}
% Here, $\calL_{m}$ is the mixing loss, $\calL_{c}$ is the classifier loss and $\calL_{d}$ is the discriminator loss.
\paragraph{Optimization Strategy.} We find that optimizing the cost function described above turns out to have slow convergence.
In order to speed up convergence, we add a more direct and explicit parameterization to the latent space. Now, the update strategy consists of two parts. Firstly, backpropagation works towards ensuring the soft constraint is satisfied. Second, the hard constraint imposed by constraining the representation as a point on a Stiefel manifold i.e. $\calS_{d,k} =\{\bU \in \bbR^{d \times k}:\bU^\top\bU  = \bI\}$, helps push the convergence along. We note that the hard constraint is only applied during training, and not at test-time. We utilize the Cayley transformation that has been widely used in manifold optimization techniques. The differentiability of this transformation allows the gradient information to backpropagate through this transformation. Given a skew symmetric matrix $\bA$, the Cayley update with a step size $\tau$ is given by:
\begin{align}
    \bZ_{new} = \big(\bI +\frac{\tau}{2}\bA\big)^{-1}(\bI - \frac{\tau}{2}\bA) \bZ,
\end{align}
where, $\bA = \bJ \bZ^\top - \bZ \bJ^\top$ where, $\bJ$ is the Jacobian with respect to the objective function.


==> Sections/SAP.tex <==
\begin{table}[h!]
{\small 
\centering
\begin{tabular}{|l|c|c|c|c|c|c|c|}
\hline
Dataset & MIX & \textbf{POS} + MIX & $\beta$-VAE & \textbf{POS} + $\beta$-VAE & Factor-VAE & \textbf{POS} + Factor-VAE\\
\hline\hline
2D Sprites & 39.6 & 40.0 & 40.3 & 40.9 & 40.7 & 41.0 \\
CelebA & 26.0 & 26.3 & 25.7 & 25.9 & 25.9 & 26.3 \\
\hline
\end{tabular}
\caption{SAP Score values for different datasets with various approaches with and without \textbf{POS} parameterization.}
\label{table:sap}
}
\end{table}

==> Sections/celeba_grid.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=2cm]{images/grid/celebA/moustache_bad.jpg}
\includegraphics[width=2cm]{images/grid/celebA/moustache_good.jpg}
\hspace{0.1cm}
\includegraphics[width=2cm]{images/grid/celebA/complexion_bad.jpg}
\includegraphics[width=2cm]{images/grid/celebA/complexion_good.jpg}
\hspace{0.1cm}
\includegraphics[width=2cm]{images/grid/celebA/hair_bad.jpg}
\includegraphics[width=2cm]{images/grid/celebA/hair_good.jpg}
   \caption{Results showing improvement over \cite{Mixing_2018} (left in each pair) with \textbf{PrOSe} (right in each pair) for three factors:  Moustache (Pair 1), Complexion (Pair 2) and Hair (Pair 3) for CelebA face dataset.The top row denotes the factor to be transferred and the right column represents the original image.}
\label{fig:celeba_grid}
\end{figure}

==> Sections/clustering.tex <==
\begin{table}[h!]
{\small 
\centering
\begin{tabular}{|l|c|c|}
\hline
Dataset & MIX & \textbf{POS} + MIX\\
\hline\hline
MNIST & 47.8 & 80.1 \\
2D Sprites & 24.5 & 99.8 \\
\hline
\end{tabular}
\caption{NMI Score values for different datasets with various approaches with and without \textbf{POS} parameterization.}
\label{table:clustering}
}
\end{table}

==> Sections/interpolation_beta_factor.tex <==
% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=6cm, height=6cm]{images/Beta_VAE/fixed_img_before.jpg}
% \includegraphics[width=6cm, height=6cm]{images/Beta_VAE/fixed_img_after.jpg}
% \hspace{2cm}
% \includegraphics[width=6cm, height=6cm]{images/Factor_VAE/factor_before.jpg}
% \includegraphics[width=6cm, height=6cm]{images/Factor_VAE/factor_after.jpg}
% \end{center}
%   \caption{Interpolation across each of the dimensions of $\beta$-VAE \cite{Matthey2017betaVAELB} with (Right) and without (Left) imposed orthogonality constraint for 2D Sprites dataset, each row representing different dimensions of the latent space.}
% \label{fig:beta_VAE_factor_VAE}
% \end{figure}

\begin{figure}[h]
\begin{center}
\includegraphics[width=12.5cm, height=6cm]{images/Beta_VAE/sprites.png}
%\includegraphics[width=13cm, height=6cm]{images/Factor_VAE/celebA.png}
\end{center}
   \caption{Interpolation across each of the dimensions of latent space: For 2D Sprites $\beta$-VAE (left) and \textbf{PrOSe} + $\beta$-VAE (right).}
\label{fig:beta_VAE}
\end{figure}



==> Sections/interpolation_mnist.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=6cm]{images/interpolation/angle_bad.jpg}
\includegraphics[width=6cm]{images/interpolation/angle_good.jpg}
\includegraphics[width=6cm]{images/interpolation/width_bad.jpg}
\includegraphics[width=6cm]{images/interpolation/width_good.jpg}
\includegraphics[width=6cm]{images/interpolation/id_bad.jpg}
\includegraphics[width=6cm]{images/interpolation/id_good.jpg}
\end{center}
   \caption{Interpolation across disentangled individual partitions signifying different attributes: Angle (Row 1), Stroke Width (Row 2), Identity (Row 3) with (Right) and without (Left) imposed orthogonality constraint for MNIST dataset.}
\label{fig:interpolation_mnist}
\end{figure}

==> Sections/interpolation_sprites.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=6.3cm]{images/interpolation/hair_sprites_bad.jpg}
\includegraphics[width=6.3cm]{images/interpolation/dress_sprites_bad.jpg}
\includegraphics[width=6.3cm]{images/interpolation/hair_sprites_good.jpg}
\includegraphics[width=6.3cm]{images/interpolation/dress_sprites_good.jpg}
\end{center}
\vspace{-0.5cm}
   \caption{Interpolation in the code vector for 2 different disentangled attributes: Hair (Left) and Armour (Right) for \cite{Mixing_2018} (Top) and \textbf{PrOSe}  (Bottom).}
\label{fig:interpolation_sprites}
\end{figure}


==> Sections/map_new.tex <==
%\begin{wraptable}{r}{0.7\textwidth}
\begin{table}[h!]
{\small 
\centering
	{\fontsize{8}{9}\selectfont
\begin{tabular}{|l|c|c|c|c|c|c|c|}
\hline
Method & Body & Skin & Vest & Hair & Arm & Leg & Avg.\\
\hline\hline
With Cayley & 70.1 & 75.5 & 88.5 & 63.2 & 72.1 & 94.4 &  77.3\\
Without Cayley & 71.2 & 74.8 & 88.2 & 62.9 & 71.6 & 95.5 & 77.4\\\hline\hline
\hline
\end{tabular}
}
\caption{mAP values for different attributes for 2D Sprites with and without Cayley Transformation step.}
\label{table:map}
}
\end{table}
%end{wraptable}



==> Sections/mnist_grid.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=2cm]{images/grid/without_identity.jpg} 
\includegraphics[width=2cm]{images/grid/with_id.jpg}
\hspace{0.17cm}
\includegraphics[width=2cm]{images/grid/without_nothing.jpg}
\includegraphics[width=2cm]{images/grid/with_angle.jpg}
\hspace{0.17cm}
\includegraphics[width=2cm]{images/grid/without_strokewidth.jpg}
\includegraphics[width=2cm]{images/grid/with_stroke_width.jpg}
   \caption{Results showing improvement over \cite{Mixing_2018} (left in each pair) with \textbf{PrOSe} (right in each pair) for three factors: Identity (Pair 1), Slant Angle (Pair 2) and Stroke Width (Pair 3) for MNIST dataset. The top row denotes the factor to be transferred and the right column represents the original image.} 
\label{fig:mnist_grid}
\end{figure}


==> Sections/predicted_mnist.tex <==
\begin{figure}[h!]
\begin{center}
\includegraphics[width=1.5cm]{images/prediction_model/actual_id.jpg}
\includegraphics[width=1.5cm]{images/prediction_model/predicted_id.jpg}
\hspace{2cm}
\includegraphics[width=1.5cm]{images/prediction_model/actual_id_after.jpg}
\includegraphics[width=1.5cm]{images/prediction_model/predicted_id_after.jpg}
\end{center}
   \caption{Prediction model trained for predicting identity for MNIST (Row 1) and hair colour for 2D Sprites (Row 2) using remaining attribute code vectors. Col 1 and 3 depict the original reconstructed batches while Col 2 and 4 represent the predicted batches with (Col 4) and without (Col 2) imposed orthogonality constraint.}
\label{fig:prediction_model_mnist}
\end{figure}

==> Sections/predicted_sprites.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=3cm]{images/prediction_model/actual_sprites_without.jpg}
\includegraphics[width=3cm]{images/prediction_model/predicted_sprites_without.jpg}
\hspace{0.5cm}
\includegraphics[width=3cm]{images/prediction_model/actual_sprites_with.jpg}
\includegraphics[width=3cm]{images/prediction_model/predicted_sprites_with.jpg}
\end{center}
   \caption{Prediction model for the hair colour attribute over 2D Sprites dataset. Col 1 and 3 depict the original reconstructed batches while Col 2 and 4 represent the predicted batches with (Col 4) and without (Col 2)\textbf{PrOSe}.}
\label{fig:prediction_model_sprites}
\end{figure}

==> Sections/sprites_grid.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=2cm]{images/grid/sprites/complexion_plus_pose_without.jpg}
\includegraphics[width=2cm]{images/grid/sprites/complexion_with_final.jpg}
\hspace{0.1cm}
\includegraphics[width=2cm]{images/grid/sprites/hair_pose_without.jpg}
\includegraphics[width=2cm]{images/grid/sprites/hair_with.jpg}
\hspace{0.1cm}
\includegraphics[width=2cm]{images/grid/sprites/vest_plus_legcolor_without.jpg}
\includegraphics[width=2cm]{images/grid/sprites/vest_color_with.jpg}
\end{center}
  \caption{Results showing improvement over \cite{Mixing_2018} (left in each pair) with \textbf{PrOSe}  (right in each pair) for three factors: Complexion (Pair 1), Hair colour (Pair 2) and armour colour (Pair 3) for 2D Sprites dataset. The top row denotes the factor to be transferred and the right column represents the original image.}
\label{fig:sprites_grid}
\end{figure}


==> Sections/tsne_mnist_id.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=4cm, height=3cm]{images/tsne/mnist_identity_tsne_without_new.png}
\hspace{1cm}
\includegraphics[width=4cm, height=3cm]{images/tsne/mnist_identity_tsne_with_new.png}
\end{center}
   \caption{t-SNE Plots for Identity Space for MNIST dataset with MIX (left) and \textbf{PrOSe} +MIX (right). The different colors denote different digit class spaces.}
\label{fig:tsne_identity}
\end{figure}

